Rethinking Nearest Neighbors for Visual Classification

Neural network classifiers have become the de-facto choice for current "pre-train then fine-tune" paradigms of visual classification. In this paper, we investigate k-Nearest-Neighbor (k-NN) classifiers, a classical model-free learning method from the pre-deep learning era, as an augmentation to modern neural network based approaches. As a lazy learning method, k-NN simply aggregates the distance between the test image and top-k neighbors in a training set. We adopt k-NN with pre-trained visual representations produced by either supervised or self-supervised methods in two steps: (1) Leverage k-NN predicted probabilities as indications for easy vs. hard examples during training. (2) Linearly interpolate the k-NN predicted distribution with that of the augmented classifier. Via extensive experiments on a wide range of classification tasks, our study reveals the generality and flexibility of k-NN integration with additional insights: (1) k-NN achieves competitive results, sometimes even outperforming a standard linear classifier. (2) Incorporating k-NN is especially beneficial for tasks where parametric classifiers perform poorly and / or in low-data regimes. We hope these discoveries will encourage people to rethink the role of pre-deep learning, classical methods in computer vision. Our code is available at: https://github.com/KMnP/nn-revisit.

==> main/table_setup.tex <==
\begin{table}
% \small
\scriptsize
\begin{center}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l  l}
\Xhline{0.7pt}\noalign{\smallskip}
\textbf{Types} &\textbf{Details}
\\
\Xhline{0.7pt}\noalign{\smallskip}
% \parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{\multirow{4}{*}{\rn-50} }}}

\textbf{Pre-trained Objective}  &\suplong{} (\supshort{}) \\ &Self-supervised: \\

&\quad 
\mocotwo{}~\cite{he2020moco,chen2020mocov2},
\moco{}~\cite{chen2021mocov3}, 
\\
&\quad 
\swav{}~\cite{caron2020swav}, 
\btwins{}~\cite{zbontar2021barlow},
\\
&\quad 
\simclr{}~\cite{chen2020simclr}, 
\dino{}~\cite{caron2021dino},
\moby{}~\cite{xie2021moby}
\\

\hline\noalign{\smallskip}

\textbf{Pre-trained Dataset} 
&
\imagenet{}~\cite{imagenet_cvpr09}, 
\inatlong{} (\inat{})~\cite{VanHorn2021newt}
\\

\hline\noalign{\smallskip}

\textbf{Backbone} 
&\rn{}-$\{$18, 50, 101, 152$\}$~\cite{he2016rn},
\\
&\vit{}-$\{$S/16, B/16, L/16$\}$~\cite{dosovitskiy2020vit}, 
\\
&\swin{}-$\{$T, S, B$\}$~\cite{liu2021swin} 
\\
\Xhline{0.7pt}\noalign{\smallskip}
\end{tabular}
}%resize
\caption{Specifications of the feature representation included in Sec.~\ref{sec:exp} and~\ref{sec:ana}.}
\label{tab:setup}
\end{center}
\end{table}
